Ferroelectric thermal phase transition and polarization precursor dynamics in CaxBa1-xNb2O6(CBN) tungsten bronze type oxides

Polycrystals of CaxBa1-xNb2O6(CBN) tungsten bronze type oxides have been prepared and their structural, dielectric, and thermal properties have been investigated. It was found that CBN alloys with ferroelectric tetragonal tungsten bronze structure were only available in a composition range of 0.19 <= x <= 0.32. It was also showed that CBN can be classified as a ferroelectric with a first-order thermal phase transition showing polarization precursor dynamics before transition into the ferroelectric phase, in sharp contrast to an isostructural alloy SrxBa1-xNb2O6(SBN) that shows typical relaxor behaviors. The local polarizations were found to grow exponentially within the paraelectric mother phase in a large temperature range of Tc<T<Tc+ 88~140 K on cooling. Furthermore, a phase diagram was established for CBN ferroelectric alloys. These findings may get an insight into the true nature of ferroelectric phase transition in this potential electro-optic material.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

